Renormalization group study of superfluid phase transition: effect of compressibility

Dynamic critical behavior in superfluid systems is considered in a presence of external stirring and advecting processes. The latter are generated by means of the Gaussian random velocity ensemble with white-noise character in time variable and self-similar spatial dependence. The main focus of this work is to analyze an effect of compressible modes on the critical behavior. The model is formulated through stochastic Langevin equations, which are then recast into Janssen-De Dominicis response formalism. Employing the field-theoretic perturbative renormalization group method we analyze large-scale properties of the model. Explicit calculations are performed to the leading one-loop approximation in the double $(\varepsilon, y)$ expansion scheme, where $\varepsilon$ is a deviation from the upper critical dimension $d_c = 4$ and $y$ describes a scaling properties of the velocity ensemble. Altogether five distinct universality classes are expected to be macroscopically observable. In contrast to the incompressible case, we found that compressibility leads to an enhancement and stabilization of non-trivial asymptotic regimes.

==> intro_old.tex <==

 Non-equilibrium physics \cite{Tauber2014,HHL08} constitutes a fascinating research topic, which  has
 been thoroughly studied in last decades.  Typical non-equilibrium problems can not be usually solved 
 exactly.  However, certain amount of simplification is possible near continuous phase transitions, where 
 many strongly interacting microscopic degrees of freedom behave in a correlated fashion  over largely 
 separated spatial scales. This results in a dynamically generated symmetry known as scale invariance~\cite{cardy}. 
 System effectively forgets microscopic details and it is then sufficient to concentrate  only on a behavior of a 
 few coarse grained macroscopic quantities. These correspond to slow modes of the system and are dictated by appropriate
 conservation laws.
 
The liquid-vapor critical point, $\lambda$-transition in superfluid helium  $\mbox{}^4$He and transition between 
ferromagnetic and paramagnetic phase near Curie temperature belong to famous examples of continuous phase transitions
\cite{Zinn}. From an experimental point of view \cite{Folk06}, distinguished role is played by the phase transition of
$\mbox{}^4$He in which
the critical region is experimentally accessible better than in any other experimental system. Sophisticated
techniques have to be applied in order to overcome slow dynamic transients. Interests {in} the theoretical investigation
of Bose-con\-den\-sa\-tes in {the} superfluid state retrieved anew interest after recent experimental achievements in 
con\-den\-sa\-tion of diluted inert gases \cite{gas}. Superfluidity emerges at $\lambda-$point, where the viscosity of 
the fluid vanishes \cite{Barenghi08,Altland}. Let us note that the critical dimension of {the} viscosity coefficient, i.e. 
the law defining  its behavior in the limit $\nu\rightarrow 0$, is not yet fully determined. This drawback might be explained 
by the fact that traditionally the critical 
dynamics in the vicinity of the lambda point is described {by} model E or F in the standard terminology \cite{HH77,Tauber2014}. 
In the  framework of {a} traditional  construction of aforementioned models, the velocity, whose dynamics is described
by the Navier-Stokes equation, is infrared   (IR) irrelevant. As a result, the vis\-co\-si\-ty  drops out of theoretical
description and therefore can not be studied.  

%------------------------------------------------------------------------------------------%
%			Inherent problems
%-----------------------------------------------------------------------------------------
In a critical region the correlation length is divergent. Due to the small value of viscosity any small velocity fluctuation
can be considerably enhanced and thus large Reynolds numbers are  expected. According to Kolmogorov hypothesis
\cite{Kolmogorov1,Kolmogorov2} there exists an inertial interval in which transfer of energy from large to small scales 
takes place and in this interval homogeneous isotropic turbulence is realized. It is assumed that there is large scale
behavior of the fluid near the outer boundary of the system \cite{Frisch}. One can
imagine that some large vortex of the system size is created, i.e., that energy is pumped into a system at very large
spatial scales. The injected energy is then transported via non-linearities in Navier-Stokes equation from the outer to
smallest scales. This transport takes place in aforementioned inertial interval where scaling behavior is present 
\cite{Frisch,Davidson}. In what follows we utilize the perturbative renormalization group (RG) technique in order to
gain information about the way external velocity fluctuations might affect the critical behavior  model E. 
%=======================================================================================================================
 
Superfluid phase transition with inclusion of velocity fluctuations and also in compressible turbulent flows was studied 
in the past as well \cite{Folk06,ivanov}. Model E and F of critical dynamics with an activated hydrodynamic modes were
proposed and investigated within the means of the RG method for the incompressible fluid in \cite{krasnov,TMF13,PRE16}.
However, it has been shown that hydrodynamic fluctuations contribute significantly to the value of the $\omega$-index,
 which is important for an overall stability analysis. The behavior of a real system near its critical point is extremely 
sensitive to external disturbances, geometry of
the experimental setup, gravity, presence of impurities and so on \cite{ivanov}. Therefore, it is important to study a
possible deviation from the ideal situation. The main aim of the present work is to determine whether presence of 
compressibility can lead to new effects in comparison with the incompressible case. Moreover some disturbances (randomly
distributed impurities or turbulent mixing) can generate completely new types of critical behavior with rich and rather
exotic properties, e.g. expansion in $\sqrt[]{\varepsilon}$ rather than in $\varepsilon$, where $\varepsilon$ is a deviation 
from the upper critical dimension $4$, i.e. $\varepsilon=4-d$. \cite{KH, JOS, SR, SR1}. Investigation of the effects of
various kinds in deterministic or chaotic flows (laminar shear flows, turbulent convection and so on) on the behavior of the 
critical fluids (like binary liquid mixtures near their consolution points) has shown that the flow can destroy the usual
critical behavior, typical of the $\varphi^4$ or Reggeon models. There can be a change to the mean-field behavior or, under some
conditions, to a more complex behavior described by new non-equilibrium universality classes.

In general terms, the fluid dynamics is governed by the Navier-Stokes equation \cite{Landau_fluid}. A formidable task of 
finding its solution remains one of the last unsolved classical problems \cite{Frisch}. In contrast to the 
mathematics, physicist's approach to turbulence follows a different path. Instead of considering a difficult mathematical 
problem 
 related to boundary and initial conditions, their effect is replaced by properly chosen random force. The resulting 
 Navier-Stokes equation is amended by an additive random variable, which also mimics a continuous input of the energy into the 
 system. Such approach has been employed in the past, and  explains many processes in turbulent flows
 \cite{turbo,Frisch,pismak,Davidson}.  Despite its success there also exists a different 
 approach, whose main idea is to model velocity fluctuations through a suitable random variable with prescribed statistical
 properties. In the literature it is known as the Kraichnan model with its various generalizations
 \cite{Kraichnan68,turbo,Ant06,FGV01,HHL16}.
  
Naively, basic premises of Kraichnan-like models can be considered as too crude. Nevertheless, important effects of 
parity breaking, anisotropy, or compressibility are easily incorporated.
Moreover, there are certain advantages from a theoretical point of view such as availability of exact solutions, and 
feasibility to compare different methods. From a practical point of view, it is intriguing that genuine properties of 
the advection problem can be captured within simplified Kraichnan-like models. 

In the original formulation of Kraichnan model, the velocity field is taken to be Gaussian, isotropic, incompressible 
and decorrelated in time. More realistic models should involve anisotropy, compressibility and finite correlation time 
\cite{Ant06}. The recent studies have pointed out some significant differences between the zero and finite correlation 
time problems \cite{falko, eyink, Ant00} and between the compressible and incompressible cases \cite{verga, AdzAnt98}. 
To model the turbulent mixing, we use Kraichnan rapid-change ensemble
\cite{Kraichnan68}: time-decorrelated Gaussian velocity field with the pair velocity function of the form 
$\langle vv \rangle \propto \delta(t-t') k^{-d - y}$, where $k$ is the wave number and $0<y<2$ is a free parameter with 
the realistic (“Kolmogorov”) value 
 %$y=\frac{4}{3}$.
 $y= 4 / 3$.
 This model has attracted a lot of attention in the past mainly because 
of the insight it offers
into the origin of intermittency and anomalous scaling in the fully developed turbulence~\cite{FGV01}. 
In the context of our study it is 
worth mentioning that the Kraichnan ensemble allows a straightforward incorporation of compressibility, which appears rather 
difficult if the velocity is modeled by dynamical equations. It is possible to directly generalize the Kraichnan 
ensemble to the case of finite correlation time; see, e.g., \cite{Ant99, AAH02, Ant00} for the passive scalar and \cite{AHHJ03} 
for the passive vector fields. 

%------------------------------------------------------------------------------------------%
%			Remarks on the previous work
%-----------------------------------------------------------------------------------------
Let us recall specific properties of critical behavior in model E. 
 There exist two RG fixed points in the dynamic model~E, which
are candidates to the {possible IR stable regimes} (see, e.g., \cite{Folk06,Tauber2014,Vasiliev}).
On the one hand,  two-loop calculations 
\cite{Dominicis}  do not offer decisive conclusion about the true fixed point due to a lack of accuracy in the $\upomega$ 
calculation. On the other hand, the value of the $\upomega$ index depends on the chosen dynamic model. For the same fixed
point the $\upomega$ value obtained in the framework of model F can 
differ from the analogous $\upomega$ in model E. Moreover, an inclusion of hydrodynamic
{fluctuations} can enhance this difference. 
   
%----------------------------------------------------------------------------------
A phenomenon of turbulence has been also discovered and lately analyzed in other than its original (classical) context. Among 
others we mention high energy physics \cite{AM06,MSW07,Khach08,Scheffler09,BSS09,BS11,Schlichting12,BSSV14}, quantum
turbulence \cite{Vinen02,Vinen06,KT07,SS12,BSS14}, ultracold gas \cite{NSSG12} and even inflation cosmology
\cite{MT04,BTW06,VPS10}. Due to a progress in experimental methods the case of quantum turbulence has been studied 
also directly \cite{Raman99,WG08,Bradley08,Salort}. For a turbulence in superfluids the quantum effects are of utmost
importance. From a theoretical point of view the zero temperature (ground state) of bosonic superfluid is well described 
by the non-linear Schr\"odinger equation, also known as Gross-Pitaevskii equation \cite{Gross61,Pitaevskii61}. Different 
theoretical techniques  \cite{Nemirovskii13} are available in order to study quantum turbulence and various
aspects in connection with
turbulence were recently analyzed \cite{KT07,NSG11,SNG12,MGP14}. A common feature of all these studies is a concentration 
on the quantum state of the superfluid state and thus operate well below the critical temperature. We would like to point
out that our aim here is to study behavior of phase transition in liquid helium above and close to a critical 
temperature, where all quantum effects can be neglected.  

%------------------------------------------------------------------------------------------%
%			Our aim and critical dynamics
%------------------------------------------------------------------------------------------%
The outline of the paper is as follows. In the Sec.~\ref{sec:problem} we introduce a coarse-grained formulation of the
problem, which we reformulate in terms of the field-theoretic model. Sec.~\ref{sc:renormalization} is reserved for a 
discussion of renormalization procedure.
In Sec.~\ref{sec:regimes} detailed analysis of fixed points' structure is given. Sec.~\ref{sec:crit_dim} is reserved
for a calculation of experimentally relevant critical exponents.  Main results are summarized in Sec.~\ref{sec:conclusion}. 
Supplementary sections \ref{sec:app_feynman},\ref{sec:app_anomdim} and \ref{app:coord} contain technical details of RG calculations.

